Charge-to-spin conversion in twisted graphene/WSe$_2$ heterostructures

We investigate the twist angle dependence of spin-orbit coupling (SOC) proximity effects and charge-to-spin conversion (CSC) in graphene/WSe$_2$ heterostructures from first principles. The CSC is shown to strongly depend on the twist angle, with both the spin Hall and standard Rashba-Edelstein efficiencies optimized at or near 30{\deg} twisting. Symmetry breaking due to twisting also gives rise to an unconventional Rashba-Edelstein effect, with electrically generated non-equilibrium spin densities possessing spins collinear to the applied electric field. We further discuss how the carrier doping concentration and band broadening control the crossover between the Fermi-sea and -surface spin response, which reconciles the seemingly disparate experimental observations of different CSC phenomena.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
